Situated Ground Truths: Enhancing Bias-Aware AI by Situating Data Labels with SituAnnotate

In the contemporary world of AI and data-driven applications, supervised machines often derive their understanding, which they mimic and reproduce, through annotations--typically conveyed in the form of words or labels. However, such annotations are often divorced from or lack contextual information, and as such hold the potential to inadvertently introduce biases when subsequently used for training. This paper introduces SituAnnotate, a novel ontology explicitly crafted for 'situated grounding,' aiming to anchor the ground truth data employed in training AI systems within the contextual and culturally-bound situations from which those ground truths emerge. SituAnnotate offers an ontology-based approach to structured and context-aware data annotation, addressing potential bias issues associated with isolated annotations. Its representational power encompasses situational context, including annotator details, timing, location, remuneration schemes, annotation roles, and more, ensuring semantic richness. Aligned with the foundational Dolce Ultralight ontology, it provides a robust and consistent framework for knowledge representation. As a method to create, query, and compare label-based datasets, SituAnnotate empowers downstream AI systems to undergo training with explicit consideration of context and cultural bias, laying the groundwork for enhanced system interpretability and adaptability, and enabling AI models to align with a multitude of cultural contexts and viewpoints.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> samples/case_study.tex <==

\section{Case Study: Image Annotation Situations}
\label{cv}


\subsection{SituAnnotate Customization and Querying}


SituAnnotate offers flexibility by allowing specialization for specific annotation situations types. For instance, we can specialize into an Image Annotation Situation (IAS) module (see Figure \ref{fig:ias}) designed to capture nuances in image annotations. For example, Figure \ref{fig:abox} illustrates how SituAnnotate can clarify and enrich the annotation of an image with the label "impressionism," detailing the context of such an annotation. This includes the explicit tracking of the fact that the label was assigned by an \textit{ArtificialAnnotator} with a vision transformer \textit{ModelArchitecture}, pretrained on the artbench-10 \textit{Database}. 

\begin{figure*}[h]
  \includegraphics[width=\textwidth]{img/ias_tbox.png}
  \caption{Specialization of the SituAnnotate pattern specifically for Image Annotation Situations, which are crucial in the field of Computer Vision (CV). Further specializations can be performed modularly, to include details specific to certain types of annotation situations (e.g., object detection situations).}
  \label{fig:ias}
\end{figure*}


\begin{figure*}[h]
  \includegraphics[width=\textwidth]{img/abox.png}
  \caption{An example use of the ImageAnnotationSituation specialization, in which the contextual situation in which the label "impressionism" was attached to a specific image can be formally represented.}
  \label{fig:abox}
\end{figure*}
% \subsection{Image Annotation Situation}

% \begin{figure*}
%   \includegraphics[width=\textwidth]{img/situannotate-cv.png}
%   \caption{The bla bla.}
%   \label{fig:teaser}
% \end{figure*}



% \subsubsection{Motivation}

% Traditional image annotation pipelines often treat semantic labels as objective facts, without accounting for the subjective and culturally-coded elements that influence the annotation process. Images, especially cultural artifacts, convey meaning not only through their raw features but also through the cultural and social contexts in which they are interpreted \citep{barthes1981camera}. The assignment of semantic labels to images can be culturally biased, leading to the reinforcement of specific interpretations and visions of the world.

% The IAS ontology module aims to address these challenges by explicitly representing the annotation context and capturing the cultural aspects of image interpretation. By doing so, it promotes transparency, interpretability, and ethical considerations in AI data labeling.

% \subsubsection{Modeling Image Annotation Situations}




% Influenced by the work in \cite{vacura2008describing}, in the IAS module we consider that the image annotation process is a situation (i.e. a context reified in the class \texttt{ImageAnnotationSituation}) that needs to be described via an \texttt{ImageAnnotationDescription}, and that represents the state of affairs of all entities related to that state of affairs: the actual \texttt{Image} to be annotated, the \texttt{Annotator} and information related to them, the time and place of the annotation situation, whether and how the annotator was remunerated, whether the annotation was done for the creation of a specific dataset, etc. The \texttt{ImageAnnotationSituation} class applies the Situation pattern to allow the contextualization of things that have something in common, or are associated: a same place, time, view, causal link, systemic dependence, etc. In the case of IAS, an \texttt{ImageAnnotationSituation} provides a context and is the setting for a variety of things that share a same informational space. In Figure~\ref{fig:MIAM_TBox}, IAS and its representation of culturally-coded annotation contexts are shown.

% The IAS module not only allows the explicit integration of cultural contextual information regarding image annotation situations, but also provides the infrastructure to \textit{compare} different image annotation situations connected to the same image object. In other words, an IAS-based knowledge graph (see Figure~\ref{fig:MIAM_ABox}) can be SPARQL queried in order to retrieve all the \texttt{ImageAnnotationSituation}s that an image may be involved in, and more specific queries can be performed to compare and better understand the contexts in which (potentially contradictory) interpretations of the same image, or parts of it, were produced.

% In the IAS module, an \texttt{ImageAnnotationSituation} is represented as a non-physical object, contextualizing the process of annotating an image. It captures relevant information such as the image to be annotated, the annotator involved, the time and place of annotation, remuneration details, the purpose of the annotation, and any cultural or bias-aware guidelines provided to the annotator.

% The use of the Descriptions and Situations (DnS) ontology pattern \citep{gangemi2003understanding} in the IAS module allows for a first-order manipulation of theories and models, enabling the representation of complex, non-physical entities like image annotation situations. DnS provides the framework to express how the intended meaning of the annotation results from statements and assertions made during the annotation process.

% \subsubsection{Comparing Annotation Situations}

% One of the key features of the IAS module is the ability to compare different \texttt{ImageAnnotationSituation}s associated with the same image or set of images. By representing different contexts and perspectives, it becomes possible to identify potential discrepancies in interpretations and understand how cultural biases and situational factors may influence the resulting semantic labels.

% The IAS-based knowledge graph allows for SPARQL queries that retrieve all \texttt{ImageAnnotationSituation}s an image may be involved in. Researchers and developers can perform more specific queries to analyze and compare the annotations, gaining valuable insights into the variations and sources of bias in the labeled data.

% \subsubsection{Enhancing AI Interpretability}

% Incorporating the IAS module into the computer vision pipeline enhances AI interpretability by providing a more comprehensive understanding of the labeled data. The explicit representation of annotation contexts and the tracking of culturally-coded annotation situations allow AI developers to critically analyze potential biases and make informed decisions about data suitability.

% Furthermore, the IAS module fosters transparency in the AI decision-making process by acknowledging the subjectivity of image annotation and the influence of cultural factors. By promoting responsible data labeling practices, it helps mitigate bias and ensures the development of more ethical and fair AI models.

% \subsection{Other Specializations}

% \begin{figure*}
%   \includegraphics[width=\textwidth]{img/situannotate-dl.png}
%   \caption{The bla bla.}
%   \label{fig:teaser}
% \end{figure*}

% Apart from the Image Annotation Situation, SituAnnotate supports various other specialized modules to represent context-aware annotations for different domains and applications. These specializations can capture the nuances of specific annotation processes, including text annotation, audio annotation, medical image annotation, and more.

% Each specialized module within SituAnnotate shares the core principles of context-aware representation and ethical considerations. The ontology provides a flexible and extensible framework for researchers and developers to adapt and apply context-aware annotations to a wide range of AI tasks and datasets.

% In summary, SituAnnotate's specializations, such as the Image Annotation Situation, pave the way for a new era of context-aware AI data labeling. By acknowledging the cultural aspects and situational influences in the annotation process, SituAnnotate enables more transparent, interpretable, and ethical AI decision-making across various domains.

% % \section{Use Case: Enhancing AI Interpretability in Computer Vision}
% %    \subsection{Case Study 1: Contextual Knowledge Capture in Computer Vision Pipelines}
% %       \subsubsection{Methodology and Data Collection}
% %       \subsubsection{Application of SituAnnotate in the Computer Vision Pipeline}
% %       \subsubsection{Analysis of Results and Impact on AI Interpretability}

% % \section{Use Case: Multilingual Knowledge Representation}
% %    \subsection{Case Study 2: Capturing Multilingual Knowledge from Corpus Linguistics}
% %       \subsubsection{Research Objectives and Data Selection}
% %       \subsubsection{Implementing SituAnnotate for Multilingual Knowledge Representation}
% %       \subsubsection{Evaluating the Effectiveness of SituAnnotate in Linguistic AI Applications}



% % \section{Case Studies}
% %     \subsection{Case Study 1: Contextual Knowledge Capture in Computer Vision Pipelines}
% %         \subsubsection{Methodology and Data Collection}
% %         \subsubsection{Application of SituAnnotate in the Computer Vision Pipeline}
% %         \subsubsection{Analysis of Results and Impact on AI Interpretability}
% %     \subsection{Case Study 2: Capturing Multilingual Knowledge from Corpus Linguistics}
% %         \subsubsection{Research Objectives and Data Selection}
% %         \subsubsection{Implementing SituAnnotate for Multilingual Knowledge Representation}
% %         \subsubsection{Evaluating the Effectiveness of SituAnnotate in Linguistic AI Applications}





Rapidly expanding image collections, including visual catalogues from the Cultural Heritage field, have attracted significant research efforts for the automatic understanding, retrieval, and management of images \citep{llamas2016applying, saleh2018image, wang2021data}. Graph-based resources are used to organize and assign meaning to the raw content of images, as well as to interconnect such meanings to other images and datasets. Scene-graphs, ontologies and other graph-based linguistic resources, such as WordNet \citep{miller1995wordnet}, are considered the best models for semantically annotating complex image scenes, to support tasks such as their automatic understanding and interpretation. These models enable the extraction of fine-grained information from image collections, which is crucial for obtaining relevant semantics as well as relational information between recognized objects \citep{sager2021survey}. Some image labelling and retrieval systems rely on large, strongly connected Knowledge Graphs, such as ConceptNet \citep{liu2004conceptnet} and Framester \citep{gangemi2016framester}, to assign and/or refine the meaning of raw features of images \citep{martinez2021automatic, samih2021semantic, tariq2017learning}. In turn, these data are used to capture and organize the content of images and as ground truths for training computer vision systems.

However,  meanings assigned to images are not culturally agnostic. Rather, visual forms illustrate, and circulate, concepts both by providing links to depicted objects through raw features–such as lines, color, shape, and size–as well as through what Barthes called an image’s ‘connotation’: a second layer of meaning made from culturally coded elements \citep{barthes1981camera}. These culturally coded elements guide humans in making decisions of where to identify objects, how to label them, how to attribute features to them, and how to establish relationships between them. 

In fact, classification systems which provide ground-truth meanings to widely used repositories of images, such as ImageNet \citep{deng2009imagenet}, may stabilize contested political categories in ways that are difficult to see. For example, an image of an indigenous person wearing a traditional garment may be classified as “half naked”, or an image of a person sleeping on a bench as “homeless”. Because classification systems decide which features make a difference, if the culturally coded aspects of meaning assignment and organization are not incorporated into the representation of the knowledge itself, there is a significant pitfall of implicit bias and unawareness of how image classification systems may be echoing, amplifying, or restructuring certain interpretations, or visions, of the world. As such, the additional layer of culturally-coded interpretation demanded by visual material ought to be made explicit, instead of directly algorithmically coded.

This paper proposes an ontology-based module that specifically aims to represent the culturally-bound processes of annotating images, as a promising tool for more faithfully representing the multi-layered process of visual understanding. We propose a specialisation of the Description and Situations ontology design pattern \citep{gangemi2003understanding}, which models non-physical objects whose intended meanings results from statements, to account for 1) the explicit tracking of how meaning(s) associated to images in the annotation processes come from culturally coded annotation situations and 2) how these assignments of meaning can be compared.

\section{Motivation}

Increasingly, graph-based models are used to organize meaning of the raw content of both photographic and art images, for example in the form of scene graphs (e.g., Visual Genome \citep{krishna2017visual}) or taxonomies (e.g., the Tate collection\footnote{\url{https://github.com/tategallery/collection/issues/27}}). 
Many of these structures are used to provide labels for objects detected by an annotator--be it artificial, human, or a combination of both. These assigned labels are then integrated into graph-based structures connecting images at face value, i.e., they are treated as facts, rather than as beliefs or assertions bounded to a specific annotation context. 
% As such, the very structure of an annotation system may suggest claims to objectivity. 

However, the extraction and representation of semantic elements from visual material constitutes the construction of a code system that can--and should--be made explicit. This is because \textit{visuality}, different from the purely biological process of vision, is flexible and encompasses ``the way that we encounter, look at, and interpret images based on the social, cultural, technological, and economic conditions of their viewing'' \cite[32]{giotta2020ways}. That is, visuality is a cultural practice with a history marked by different habits or ways of seeing, as well as different types of spectators \citep{foster1988preface}.


\subsection{Cultural Biases in Computer Vision}

Importantly, the cultural-boundedness of visuality remains when images are passed through computer vision pipelines, including through the seemingly straightforward process of object detection. As argued by \citet{arnold2019distant} in their \textit{distant viewing} methodological and theoretical framework for large-scale study of visual materials, there is a code system required, which is culturally and socially constructed. As such, labelling and classification systems can act as forms of centralized power reflecting a specific group's or culture's values. 

Nevertheless, humans tend to show high confidence in the integrity and objectiveness of benchmark datasets' image labels, including a naive faith both in photographic truth and in the unretouched quality of images discovered online \citep{giotta2020ways}. This faith in the cultural agnosticism of images' semantic labeling is intricately related to the topic of machine-learning bias, currently leading to worldwide discussions on the importance of \textit{representation} in artificial intelligence systems. Practically and generally speaking, models will always incorporate some form of bias, since it is unrealistic to build a complete representation of the real world. However, images and the field of computer vision is especially vulnerable, as bias can occur in a variety of stages, from human reporting and selection bias to algorithmic and interpretation bias \citep{laranjeira2021}.

The idea that automated systems are not inherently neutral and instead reflect the priorities, preferences, and prejudices of those who have the power to mold artificial intelligence is an increasingly public topic of discussion. For example, recent works have demonstrated that the geographical sampling of Flickr images as well as the use of English as the primary language for dataset construction and taxonomy definition result in inherent cultural bias within the datasets \citep{de2019does}, with work being done to design new annotation procedures that enable fairness analysis \citep{schumann2021step}. Another example is \textit{Gender Shades}\footnote{\url{http://gendershades.org/}, \url{https://www.media.mit.edu/projects/gender-shades/overview/}} \citep{buolamwini2018gender}, an investigation from the Massachussets Institute of Technology on the false assumption of machine neutrality, and the \textit{coded gaze}--this algorithmic `way of seeing' which classifies content through researcher- and machine-labeled categories--which ``reflects both our aspirations and our limitations'' according to its coiner \citep[44]{buolamwini2017gender}.

\subsection{Identifying and Representing Cultural Bias}

The bias that is the focus of this paper is not to be confused with the bias term in machine learning models or prediction bias, which mathematically speaking is an intercept or offset from an origin. Instead, we intend cultural bias in the sense presented by \citet{APA2015cul}:

\begin{quote}
 the tendency to interpret and judge phenomena in terms of the distinctive values, beliefs, and other characteristics of the society or community to which one belongs. This sometimes leads people to form opinions and make decisions about others in advance of any actual experience with them (prejudice).
\end{quote} 

This article focuses specifically on \textit{how to technically account for the way that cultural bias permeates the moment of assigning semantic labels to pixel areas of images} during the creation of computer vision datasets. This specific moment of human-led or human-evaluated annotation is critical, as these labels become part of input data of widely used models across many different fields, and in that way the ``data itself'' can host a lot of human biases, such as stereotyping, prejudice or racism. In this sense, this paper is concerned with the intersection of cultural and \textit{measurement} bias. Measurement bias refers to faulty, low quality or unreliable measures when collecting data, such as inconsistent or unreliable labeling of samples, which can have many causes such as insufficient label options (e.g. binary gender \citep{scheuerman2019computers}) or from subjective views from labelers.


This paper acknowledges the gap of technical frameworks to concurrently model how meaning is culturally-bound and assigned, via beliefs, to raw visual content depending on the annotation situation within image annotation pipelines. It hypothesises that network-based structures can provide technical frameworks in order to mitigate harm from implicit cultural bias.

\subsection{Ontologies for Digital Hermeneutics}

Specifically, it sees the use of ontology-based representations for image label data as promising, since associating a meaning with complex scenes may require an explicit and symbolic representation of the domain of knowledge, and the ability to reason over it. As such, ontologies provide a powerful framework to address this issue for image analysis and interpretation \citep{bannour2011towards}; one of their biggest benefits is that the semantics is made explicit and allows queries to be formulated in terms of concepts and their relationships. 
% There are many ontology-driven approaches addressing the problem of image interpretation [eg., 30].

Ontologies for modeling interpretation related to cultural artifacts, including visual works of art, are more widespread. The IECA ontology\footnote{\url{https://ieca-ontology.github.io/}}provides a conceptual and ontological model to represent interpretative encounters between human observers and cultural artifacts, and to investigate the content, context, and relationships between alternative interpretations of cultural objects. A recent work by \cite{baroncini2021modelling} about modelling interpretation and meaning for art pieces, presents a data model for describing iconology and iconography. Previously, \cite{daquino2015historical} proposed the Historical Context Ontology (HiCO), an ontology aiming to outline relevant issues related to the workflow for stating, and formalizing, authoritative assertions about context information of cultural heritage artifacts. Also recently \cite{carboni2019ontological} have presented the VIR (Visual Representation) ontology, constructed as an extension of CIDOC-CRM (CIDOC Conceptual Reference Model), which sustains the recording of statements about the different structural units and relationships of a visual representation, differentiating between object and interpretative act.

% "garbage in, garbage out" principle.


\section{The IAS Ontology Module}

This paper discusses the potential of using an ontology-based technique for the explicit tracking of how meaning(s) associated to images come from culturally coded annotation situations, and of how these assignments of meaning can be compared. Our approach is based on the idea that an image's semantic labels depend upon the specific annotation situation under which it is interpreted. Specifically, the idea is that an \texttt{Image} can be involved in multiple annotation situations, which may differ on account of one or many aspects: when, where, and why they were performed, by whom, whether and how the annotator was remunerated, etc. In order to represent this model formally, we designed the \textbf{Image Annotation Situations (IAS) ontology} module, based on the Descriptions and Situations (DnS) ontology pattern \citep{gangemi2003understanding}, which supports a first-order manipulation of theories and models. DnS was chosen as a core design pattern because it allows for the modeling of non-physical objects, such as an image annotation system or situation, whose intended meaning results from statements, i.e. they arise in combination with other entities. 

\begin{figure}
% Use center to align a figure or table to the middle of the text column
\begin{center}
\includegraphics[width=0.8\linewidth]{Images/MIAM_TBox.png}
\end{center}
\caption{The IAS ontology module is aligned to and reuses patterns from DOLCE+DnS Ultralite (DUL) foundational ontology \citep{gangemi2002sweetening} in order to represent and give meaning to the culturally-bound context in which annotation data was created during an image annotation process. All un-prefixed classes belong to the namespace of the IAS ontology.}
\label{fig:MIAM_TBox}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.9\linewidth]{Images/MIAM_ABox.png}
\end{center}
\caption{Example use of the IAS module to formally represent a single image being involved in two different \texttt{ImageAnnotationSituation}s, which lead to different attributes (``almost naked'' and ``in traditional garment'') to the same area of pixels.All un-prefixed classes belong to the namespace of the IAS ontology.}
\label{fig:MIAM_ABox}
\end{figure}


Influenced by the work in \cite{vacura2008describing}, in the IAS module we consider that the image annotation process is a situation (i.e. a context reified in the class \texttt{ImageAnnotationSituation}) that needs to be described via an \texttt{ImageAnnotationDescription}, and that represents the state of affairs of all entities related to that state of affairs: the actual \texttt{Image} to be annotated, the \texttt{Annotator} and information related to them, the time and place of the annotation situation, whether and how the annotator was remunerated, whether the annotation was done for the creation of a specific dataset, etc. The \texttt{ImageAnnotationSituation} class applies the Situation pattern to allow the contextualization of things that have something in common, or are associated: a same place, time, view, causal link, systemic dependence, etc. In the case of IAS, an \texttt{ImageAnnotationSituation} provides a context and is the setting for a variety of things that share a same informational space. In Figure~\ref{fig:MIAM_TBox}, IAS and its representation of culturally-coded annotation contexts are shown.

The IAS module not only allows the explicit integration of cultural contextual information regarding image annotation situations, but also provides the infrastructure to \textit{compare} different image annotation situations connected to the same image object. In other words, an IAS-based knowledge graph (see Figure~\ref{fig:MIAM_ABox}) can be SPARQL queried in order to retrieve all the \texttt{ImageAnnotationSituation}s that an image may be involved in, and more specific queries can be performed to compare and better understand the contexts in which (potentially contradictory) interpretations of the same image, or parts of it, were produced.


\section{Conclusion}

The Image Annotation Situation (IAS) ontology module addresses cultural bias in image annotations systems by providing a graph-based technical representation of the culturally-bound process of annotating images. In doing so, it lays the ground for a more faithful representation of the multilayered process of visual understanding, and of the interpretative situations underlying widely spread computer vision pipelines. It is crucial to continue research on how image classification systems may be echoing, amplifying, or restructuring certain visions of the world, a task requiring an ongoing partnership between humanists and computational scholars.

\bibliography{references}

\end{document}




PREFIX ns1: <https://w3id.org/situannotate#>
PREFIX xsd: <http://www.w3.org/2001/XMLSchema#>
PREFIX rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>
PREFIX rdfs: <http://www.w3.org/2000/01/rdf-schema#>
PREFIX conceptnet: <http://etna.istc.cnr.it/framester2/conceptnet/5.7.0/c/en/>
PREFIX : <https://w3id.org/situannotate#>
    SELECT ?entity_type ?artstyle_label ?strength ?date ?place ?annotator ?architecture ?dataset
    WHERE {
        ?annotation a :ArtStyleAnnotation ;
            :aboutAnnotatedEntity ?:ARTstract_14978 ;
            :annotationWithLexicalEntry ?artstyle_le ;
            :isAnnotationInvolvedInSituation ?situation ;
            :hasAnnotationStrength ?strength ;
            :isClassifiedBy :detected_art_style .
    
		?artstyle_le rdfs:label ?artstyle_label .
        ?situation :onDate ?date ;
            :atPlace ?place ;
            :involvesAnnotator ?annotator ;
            :involvesDataset ?dataset .

        ?annotator :hasModelArchitecture ?architecture ;
            :pretrainedOnDataset ?pretrainedDataset .
    
    	:ARTstract_14978 a ?entity_type .
    
        FILTER NOT EXISTS {
        ?subClass rdfs:subClassOf ?entity_type .
        :ARTstract_14978 rdf:type ?subClass.
        FILTER (?subClass != ?entity_type)
    }
    }

    # Extract information from the query results
entity_type = query_results['results']['bindings'][0]['entity_type']['value'].split('#')[-1]
artstyle_label = query_results['results']['bindings'][0]['artstyle_label']['value']
strength = query_results['results']['bindings'][0]['strength']['value']
date = query_results['results']['bindings'][0]['date']['value']
place = query_results['results']['bindings'][0]['place']['value'].split('#')[-1]
annotator = query_results['results']['bindings'][0]['annotator']['value'].split('#')[-1]
architecture = query_results['results']['bindings'][0]['architecture']['value'].split('#')[-1]
dataset = query_results['results']['bindings'][0]['dataset']['value'].split('#')[-1]

# Format the output
output = f"The entity {entity_type} is an Image, which was annotated with the art style {artstyle_label} on the {date}, in {place}, by the artificial annotator {annotator}, which has a {architecture} model architecture and has been pretrained on the {dataset} dataset."
print(output)

==> samples/disc.tex <==
\section{Discussion}
\label{discussion}

The positive evaluation results highlight the robustness and power of SituAnnotate in formally representing information. These results indicate that SituAnnotate excels in several key aspects, providing significant advantages over traditional annotation methods.

\paragraph{\textbf{Contextual Precision}} SituAnnotate provides a highly nuanced and context-aware representation of annotations. By connecting annotations not only to the described entity but also to the broader situational context and the annotator involved, it enables a richer understanding of the circumstances in which annotations are made. This contextual precision is often lacking in traditional annotation approaches that focus solely on labels or strings.

\paragraph{\textbf{Semantic Enrichment and Expressiveness}} Unlike traditional annotation methods that often involve fixed annotation tasks and roles, SituAnnotate offers the flexibility of associating the same entity with multiple labels through various "AnnotationRoles." This semantic depth significantly enhances the ontology's expressiveness and precision. Annotators can provide richer and more detailed information about the same entity, enabling a more comprehensive understanding of the annotated data. This flexibility is particularly valuable when dealing with complex or multifaceted annotations. SituAnnotate can even formally represent cases in which the same entity, e.g. an image, is associated with the same label, e.g. "happiness," through various annotations fulfilling different AnnotationRoles, such as detected emotion or detected abstract concept. This semantic depth significantly enhances the ontology's expressiveness and precision

\paragraph{\textbf{Flexibility in Annotator Representation}} SituAnnotate is adaptable to various annotator types, including both artificial and human annotators. This adaptability addresses privacy concerns by allowing the aggregation of demographic data when needed. In today's diverse annotation landscape, which includes computer vision models, individual human annotators, and annotator communities, SituAnnotate ensures that all these entities can be formally represented. This reflects the multifaceted nature of modern annotation processes and supports inclusive and diverse annotation practices.

\paragraph{\textbf{Automated Reasoning and Data-Driven Decision-Making}} 
SituAnnotate's structured representation of annotation situations facilitates automated reasoning through SPARQL queries and semantic technologies. Machines can infer relationships, make connections, and retrieve information efficiently, streamlining the annotation understanding process. This automation not only saves time but also supports data-driven decision-making. Users can leverage SituAnnotate to extract valuable insights and patterns from annotated data, enabling evidence-based decisions and enhancing the utility of labeled datasets.

\paragraph{\textbf{Enhanced and User-Friendly Human Understanding}} SituAnnotate, despite its machine-readable foundation, offers a user-friendly ontological framework that remains accessible to researchers, domain experts, and annotators alike. This approach ensures that the ontology isn't confined to machines but serves as a valuable resource for human understanding. Moreover, the integration of SPARQL queries and Python scripts empowers users to effortlessly access and interpret situational knowledge tied to specific annotations. This user-friendly feature enhances transparency and facilitates comprehension, making SituAnnotate a versatile resource catering to both machine-driven AI technologies and human expertise. This symbiotic relationship fosters a deeper synergy between AI capabilities and human insights, emphasizing the ontology's significance in bridging the gap between technology and human cognition.

\paragraph{\textbf{Comparing Annotation Situations for Enhanced Understanding}} SituAnnotate's ability to represent multiple labels and annotation situations related to the same annotated object provides users with a powerful tool for enhanced understanding. Through SPARQL queries, users can retrieve all AnnotationSituations for an object, enabling detailed comparisons of potentially conflicting interpretations. This feature enhances the understanding of diverse annotation contexts and their implications, supporting better decision-making and data analysis.

\paragraph{\textbf{Mitigating Bias and Enhancing Ethical AI}} SituAnnotate serves as a robust tool in the battle against bias through its context-aware data annotation capabilities. Annotators can furnish essential details about data sources, annotator demographics, and the rationale behind labeling decisions. This wealth of contextual information empowers AI developers to scrutinize and rectify any latent biases when examining annotated data. By doing so, SituAnnotate champions transparency and fairness throughout the data annotation process. It contributes significantly to the ethical dimensions of AI development and deployment. As ethical considerations in AI data labeling take center stage, SituAnnotate stands as a pivotal asset, providing a context-aware framework for the meticulous recording and management of annotations.

\subsection{Limitations and Further Directions}

\section{Limitations}

Despite its promising capabilities, SituAnnotate does have some limitations and challenges:

\begin{enumerate}
    \item \textbf{Knowledge Representation Overhead:} While SituAnnotate offers enhanced contextual knowledge representation, this also introduces an overhead in terms of ontology creation, maintenance, and population. It may require substantial time and effort to initially set up and continuously update.

    \item \textbf{Capturing Human Subjectivity and Cultural Nuances:} One notable challenge lies in the complexity of capturing the full scope of contextual factors that affect human subjectivity and the diverse cultural nuances that can influence annotations. While SituAnnotate offers a structured framework, it does not fully capture the richness of human interpretation.

    \item \textbf{Scalability Concerns:} SituAnnotate's scalability may be a concern when applied to massive datasets, where managing a vast number of annotation situations and annotators can become unwieldy. Optimizing the ontology for large-scale applications is an ongoing challenge. This is also because the use of SPARQL queries and scripts to retrieve human-understandable explanations can be resource-intensive.

    \item \textbf{Privacy Mechanisms:} SituAnnotate's ability to address privacy concerns may require further refinement to provide more robust mechanisms for data anonymization and aggregation. Ensuring the privacy and confidentiality of sensitive data is crucial.
    
\end{enumerate}

These limitations should be considered when implementing SituAnnotate in real-world scenarios, and ongoing research and development efforts may help mitigate some of these challenges.

\section{Further Directions}

As SituAnnotate continues to evolve, there are several avenues for further research and development:

\begin{enumerate}
    \item \textbf{Usability Improvements:} Prioritize creating user-friendly tools and interfaces that simplify the process of integrating SituAnnotate into annotation workflows. Consider developing user-friendly graphical user interfaces (GUIs) for creating and querying annotations, enhancing accessibility for a broader user base.

    \item \textbf{Scalability:} Investigate methods to enhance SituAnnotate's scalability, particularly when dealing with large datasets. This may involve optimizing SPARQL queries or exploring distributed computing solutions to handle increasing volumes of data efficiently.

    \item \textbf{Enhanced Automation:} Continue to advance automation tools for generating human-readable explanations from the ontology. Explore Natural Language Processing (NLP) techniques to produce more coherent and concise explanations, reducing the need for manual intervention.

    \item \textbf{Interoperability:} Ensure that SituAnnotate remains compatible with other ontologies and standards in the data annotation and semantic web domain. Seamless integration with existing systems is essential for broader adoption.

    \item \textbf{Community Involvement:} Foster collaboration and engagement within the research community to refine and expand SituAnnotate. An active user and developer community can drive further innovation and adoption. Additionally, seek collaboration with the global research community to address cultural biases and diversify the ontology's applicability.

    \item \textbf{Ethical Considerations:} Delve into the ethical implications of SituAnnotate's real-world applications, particularly concerning privacy, bias, and transparency. Develop comprehensive guidelines and best practices for ethical annotation processes, promoting responsible AI development.

    \item \textbf{Scenarios and Use Cases:} Continue to develop and document a diverse set of real-world scenarios and use cases where SituAnnotate has demonstrated its practical value. Providing concrete examples can help potential users grasp its applicability better.

    \item \textbf{Integration with AI Systems:} Explore seamless integration possibilities of SituAnnotate with AI systems, particularly in domains like computer vision, natural language processing, and knowledge graphs. Incorporating advanced techniques for handling multi-modal data, including text, images, and videos, can broaden its applicability.

    \item \textbf{AI Ethics and Fairness:} Investigate how SituAnnotate can be integrated with emerging AI ethics and fairness frameworks. Contributing to more responsible and equitable AI development aligns with the growing importance of ethical considerations in the field.

\end{enumerate}

These directions encompass technical, usability, ethical, and collaborative aspects, ensuring that SituAnnotate remains a dynamic and relevant tool in the evolving landscape of data annotation and semantic web technologies.

==> samples/eval_cs.tex <==
\section{Evaluation}

\subsection{Evaluation Protocol}

The evaluation protocol consists of several steps aimed at assessing the performance and capabilities of the SituAnnotate system. These steps include the formulation of specialized competency questions, the creation of a toy dataset, the translation of the CQ questions into SPARQL queries, and the execution of these queries over the toy dataset.

\subsubsection{Competency Questions (CQs) SPARQL Queries}

In the context of the user requirement scenarios, we formulated a set of specialized Competency Questions (CQs). These CQs were designed to reflect the real-world information needs arising from the specific case study and scenarios presented earlier. These questions serve as a valuable tool for assessing the capabilities and performance of the SituAnnotate system in addressing practical use cases. Below, we present the list of CQs derived from our case study and scenarios:

\begin{enumerate}
    \item CQ1: Which countries have been the location of annotation situations, how many annotation situations were located in each country, and which country has been the location for the highest number of annotation situations?
    
    \item CQ2: Between the years 2020 and 2024, in which annotation situations has the image with ID "ARTstract\_14978" been involved?
    
    \item CQ3: What remuneration schemes have been used in annotation situations involving the "ARTstract" dataset?
    
    \item CQ4: What types of entities have been annotated?
    
    \item CQ5: Which images have been annotated using the lexical entry "surfboard," and what role did these annotations serve?
    
    \item CQ6: For the specific situation in which "surfboard" was used to annotate the image with ID "ARTstract\_14978," what contextual factors were associated with the annotation situation?
    
    \item CQ7: Which images have annotations classified under the role of "detected emotion" with an annotation strength exceeding 0.85, and what labels have been assigned to them?
    
    \item CQ8: What concepts type annotations about the image with ID "ARTstract\_14978"?
    
    \item CQ9: For each lexical entry (label) that the image with ID "ARTstract\_14978" was annotated with, who was the Annotator that assigned that label?
    
    \item CQ10: What types of annotations about the image with ID "ARTstract\_14978" were all done by artificial annotators with the "visual transformer" model architecture?
    
    \item CQ11: What are the caption annotations for the image with ID "ARTstract\_14978," and who are the annotators responsible for each caption annotation?
\end{enumerate}

\subsubsection{Toy Dataset Creation}

To evaluate the capabilities and performance of the SituAnnotate system, we crafted a toy dataset in the form of a Knowledge Graph (KG). This dataset emulates real-world scenarios involving multiple annotation situations for a single image, offering a comprehensive testbed for our system. The toy dataset encompasses a diverse array of annotation types, such as object detection, actions, emotions, art styles, colors, and more, all meticulously generated by distinct artificial annotators. Figure \ref{fig:toy} visually presents the selected image along with the various labels incorporated into the KG, showcasing the rich contextual data captured. To formalize the dataset, we employed the SituAnnotate ontology, ensuring the preservation of extensive information pertaining to each annotation situation. This encompassed details like geographical location, temporal specifics, annotated datasets, remuneration structures, detection criteria, and detailed annotator profiles. This rich contextual data not only enhances the semantic content of the dataset but also enables structured representation for diverse analytical purposes.

Our toy dataset is structured into two distinct Turtle (.ttl) files, each serving a unique purpose:

\textbf{1. Image Data Knowledge Graph}: This RDF file, available \href{https://github.com/delfimpandiani/situAnnotate/blob/main/tests/toy_dataset/images_kg.ttl}{here}, provides comprehensive data for a set of annotations related to a specific image (\textit{:ARTstract\_14978}). Each annotation within the dataset is associated with the annotation situation in which it took place. These annotations span various dimensions, including actions, age groups, artistic styles, colors, emotions, human presence, image captions, and objects, all linked to relevant ConceptNet concepts. Moreover, each annotation is enriched with an annotation strength value, reflecting its confidence or relevance. This data encapsulates the image's contextual information and semantic content, enabling structured and semantically rich representation for analytical purposes.
\begin{verbatim}
:14978_ARTstract_as_2023_06_26 a :ArtStyleAnnotation ;
    :aboutAnnotatedEntity :ARTstract_14978 ;
    :annotationWithLexicalEntry :le_Impressionism ;
    :hasAnnotationStrength 0.6149182915687561 ;
    :isAnnotationInvolvedInSituation :ARTstract_as_2023_06_26 ;
    :isClassifiedBy :detected_art_style ;
    :typedByConcept <http://etna.istc.cnr.it/framester2/conceptnet/5.7.0/c/en/impressionism> .

:ARTstract_14978 a :Image ;
      rdfs:comment "painting of children playing in the water at the beach"^^xsd:string ;
    :isInvolvedInAnnotationSituation :ARTstract_act_2023_06_28,
        :ARTstract_age_2023_06_26,
        :ARTstract_as_2023_06_26,
        :ARTstract_color_2023_06_26,
        :ARTstract_em_2023_06_26,
        :ARTstract_hp_2023_06_26,
        :ARTstract_ic_2023_06_28,
        :ARTstract_od_2023_06_28 .      
    :hasImageLabelTypedBy conceptnet:contentment,
        conceptnet:gray,
        conceptnet:human,
        conceptnet:impressionism,
        conceptnet:person,
        conceptnet:running,
        conceptnet:silver,
        conceptnet:surfboard,
        conceptnet:twenties ;
    :isAnnotatedWithLexicalEntry :le_20-29,
        :le_Impressionism,
        :le_True,
        :le_contentment,
        :le_dimgray,
        :le_gray,
        :le_person,
        :le_running,
        :le_silver,
        :le_surfboard ;

\end{verbatim}

\textbf{2. Annotation Situations Knowledge Graph (KG)}: This RDF file, accessible \href{https://github.com/delfimpandiani/situAnnotate/blob/main/tests/toy_dataset/situations_kg.ttl}{here}, contains detailed representations of the annotation situations themselves. It includes instances of various annotation situation types, each described with specific attributes and relationships. Notably, the KG incorporates instances of artificial annotators responsible for generating annotations. These annotators are associated with specific model architectures and datasets. The KG references datasets used in annotation situations, enhancing the context of each situation. Additionally, geographical locations of situations are represented, with instances such as \texttt{:Italy}. Model architectures used by artificial annotators are documented within the KG.
\begin{verbatim}
:ARTstract_as_2023_06_26 a :ArtStyleAnnotationSituation ;
    :involvesAnnotatedEntity :ARTstract_14978 ;
    :atPlace :Italy ;
    :hasDetectionThreshold "top_one" ;
    :involvesAnnotator :oschamp_vit-artworkclassifier ;
    :involvesDataset :ARTstract ;
    :onDate "2023-06-26"^^xsd:date ;
    :satisfies :as_detection_desc .

:as_detection_desc a ns1:ImageAnnotationDescription ;
    rdfs:comment "Art style detections are annotation situations 
        in which annotations play the role of detected_art_style, 
        assigned by an Annotator according to a certain detection 
        threshold or heuristic"^^xsd:string ;
    :defines :detected_art_style .

:oschamp_vit-artworkclassifier a :ArtificialAnnotator ;
    :hasModelArchitecture :visual_transformer ;
    :pretrainedOnDataset :artbench-10 .
\end{verbatim}

This comprehensive toy dataset serves as a valuable resource for evaluating the SituAnnotate system's effectiveness in handling diverse annotation situations and enriching semantic content.

\begin{figure*}[h]
  \includegraphics[width=\textwidth]{img/toy_dataset.png}
  \caption{Visualization of the toy dataset, showcasing the image and various labels incorporated into the KG. Each of these labels is hardcoded alongside all of the contextual information about the annotation situation that gave rise to it.}
  \label{fig:toy}
\end{figure*}






\subsubsection{Translation into and Execution of SPARQL Queries}

These CQs were subsequently translated into SPARQL queries, creating a formal means to retrieve specific information from the toy dataset. To evaluate the performance and effectiveness of the SituAnnotate system, we executed these SPARQL queries over the toy dataset. For executing the SPARQL queries, we used Ontotext GraphDB,\footnote{\url{https://graphdb.ontotext.com/documentation/10.0/index.html}} a highly efficient and robust graph database with RDF and SPARQL support. We ran GraphDB in a Docker container, as provided on Github.\footnote{\url{https://github.com/Ontotext-AD/graphdb-docker}} This platform facilitated the execution of SPARQL queries and retrieval of structured data in accordance with the SituAnnotate ontology. To provide a concise overview, Table \ref{tab:sparql} summarizes the Competency Questions (CQs) along with their corresponding SPARQL queries and whether they were successfully executed ("Pass" status) in evaluating the SituAnnotate system's performance.


\subsection{Human-Readable Explanations}

In addition to assessing the system's performance against the CQs, we aimed to harness the ontology's potential for retrieving situational knowledge regarding specific ground truths and presenting it in a readily understandable human language. To achieve this objective, we crafted a specialized SPARQL query capable of retrieving comprehensive contextual information for a given entity and label of interest. Subsequently, we developed a Python script, also available on our GitHub repository,\footnote{\url{github.com/delfimpandiani/situAnnotate/tests/}} to automatically translate the SPARQL query output into a human-readable narrative that elucidates the context surrounding the annotation. This endeavor underscores our commitment to facilitating seamless comprehension and transparency in annotation contexts. Here is the SPARQL query:

\begin{verbatim}
PREFIX xsd: <http://www.w3.org/2001/XMLSchema#>
PREFIX rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>
PREFIX rdfs: <http://www.w3.org/2000/01/rdf-schema#>
PREFIX conceptnet: <http://etna.istc.cnr.it/framester2/conceptnet/5.7.0/c/en/>
PREFIX : <https://w3id.org/situannotate#>
    SELECT ?entity_type ?strength ?date ?place ?annotator ?architecture ?dataset
    WHERE {
        ?annotation a :Annotation ;
            :aboutAnnotatedEntity :{{entity_ID}} ;
            :annotationWithLexicalEntry ?le ;
            :isAnnotationInvolvedInSituation ?situation ;
            :hasAnnotationStrength ?strength .
    
	?le rdfs:label {{label}}^^xsd:string .
        
        ?situation :onDate ?date ;
            :atPlace ?place ;
            :involvesAnnotator ?annotator ;
            :involvesDataset ?dataset .

        ?annotator :hasModelArchitecture ?architecture ;
            :pretrainedOnDataset ?pretrainedDataset .
    
    	:{{entity_ID}} a ?entity_type .
    
        FILTER NOT EXISTS {
        ?subClass rdfs:subClassOf ?entity_type .
        :{{entity_ID}} rdf:type ?subClass.
        FILTER (?subClass != ?entity_type)
        }
    }
\end{verbatim}

\subsection{Results and Online Access}

All 11 competency question verification tests were successfully passed, with the expected outcomes matching the actual results. Comprehensive details regarding the results can be accessed in our SituAnnotate GitHub repository, available at the following link: \footnote{\url{https://github.com/delfimpandiani/situAnnotate/blob/main/tests/competency_question_verification/Results.md}}. This repository provides in-depth insights into the query outcomes, presenting the retrieved information relevant to each specialized competency question. We invite readers to visit our online repository for a thorough comprehension of our evaluation process and results, facilitating further analysis as needed.

\subsection{Practical Application: Human-Understandable Explanations}

To demonstrate the practical application of SituAnnotate's capabilities, we selected an image from the toy dataset along with a random label. We executed the aforementioned SPARQL query and a Python script, which translated the query output into a human-readable explanation of the context of the annotation. Figure \ref{fig:user_query} provides an example of such an explanation for an image labeled as "impressionism." The figure showcases how the SituAnnotate ontology clarifies and enriches image annotations. It details the context of the "impressionism" label assignment, including information about the annotator, model architecture, and dataset used for training. This practical demonstration highlights the ontology's ability to provide insightful and human-understandable explanations of annotations, making it a valuable tool for situating annotations within their context.

\begin{figure*}[h]
  \includegraphics[width=\textwidth]{img/user_query.png}
    \caption{Illustration of an exemplary usage of the ImageAnnotationSituation specialization, depicting the formal representation of the contextual situation in which the label "impressionism" was assigned to a specific image. Users can employ a single SPARQL query and a small Python script to obtain fully human-understandable statements situating the ground truth label assigned to an entity, as demonstrated in this case with an image.}
  \label{fig:abox}
\end{figure*}

By combining SPARQL queries and Python scripts, we empower users to easily access and interpret situational knowledge associated with specific annotations, enhancing transparency and understanding.

\begin{landscape}
\centering
\footnotesize
\label{tab:sidewaystable}

\begin{xtabular}{|p{.8cm}|p{4cm}|p{10cm}|p{0.8cm}|}
\hline
\textbf{CQ} & \textbf{Competency Question} & \textbf{SPARQL Query} & \textbf{Pass} \\
\hline
% __________________________________________________________
CQ1 & Which countries have been the location of annotation situations, how many annotation situations were located in each country, and which country has been the location for the highest number of annotation situations? & 
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?Country (COUNT(?AnnotationSituation) AS ?count)
WHERE {
    ?AnnotationSituation :atPlace ?Country .
}
GROUP BY ?Country
ORDER BY DESC(?count)
\end{lstlisting} 
& Y \\[-5ex]
\hline
% __________________________________________________________
CQ2 & Between the years 2020 and 2024, in which annotation situations has the image with ID \textit{ARTstract\_14978} been involved? & \begin{lstlisting}[style=sparql]
SELECT ?AnnotationSituation ?Date
WHERE {
    :ARTstract_14978 :isInvolvedInAnnotationSituation ?AnnotationSituation .
    ?AnnotationSituation :onDate ?Date .
    FILTER(YEAR(?date) >= 2020 && YEAR(?date) <= 2024)
}
\end{lstlisting} 
& Y \\[-6ex]
\hline
% __________________________________________________________
CQ3 & What remuneration schemes have been used in annotation situations involving the \textit{ARTstract} dataset? & 
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?RemunerationScheme 
WHERE {
    ?AnnotationSituation rdf:type :AnnotationSituation ;
    :involvesDataset :ARTstract .
    ?AnnotationSituation :involvesRemunerationScheme ?RemunerationScheme .
}
\end{lstlisting} 
& Y \\[-10ex]
\hline
% __________________________________________________________
CQ4 & What types of entities have been annotated? & 
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT DISTINCT ?EntityType 
WHERE {
    ?Annotation :aboutAnnotatedEntity ?Entity .
    ?Entity a ?EntityType .
}
\end{lstlisting} 
& Y \\[-8ex]
\hline
% __________________________________________________________
CQ5 & Which images have been annotated using the lexical entry "surfboard," and what role did these annotations serve? & \begin{lstlisting}[style=sparql]
SELECT ?Image ?annotationRole 
WHERE {
    ?Annotation :aboutAnnotatedEntity ?Image .
    ?Annotation :annotationWithLexicalEntry :le_surfboard .
    ?Annotation :isClassifiedBy ?AnnotationRole .
}
\end{lstlisting} 
& Y \\[-5ex]
\hline
% __________________________________________________________
CQ6 & For the specific situation in which "surfboard" was used to annotate the image with ID \textit{ARTstract\_14978}, what contextual factors were associated with the annotation situation? &
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?Country ?Date ?Dataset ?RemunerationScheme ?DetectionThreshold ?Annotator ?PretrainDataset ?ModelArchitecture 
WHERE {
  ?Annotation :aboutAnnotatedEntity :ARTstract_14978 .
  ?Annotation :annotationWithLexicalEntry :le_surfboard .
  ?AnnotationSituation :involvesAnnotation ?Annotation .
  OPTIONAL {
      ?AnnotationSituation :atPlace ?Country .
      ?AnnotationSituation :onDate ?Date .
      ?AnnotationSituation :involvesDataset ?Dataset .
      ?AnnotationSituation :hasDetectionThreshold ?DetectionThreshold .
      ?AnnotationSituation :involvesAnnotator ?Annotator .
      ?Annotator :pretrainedOnDataset ?PretrainDataset .
      ?Annotator :hasModelArchitecture ?ModelArchitecture .
      ?AnnotationSituation :involvesRemunerationScheme ?RemunerationScheme .
  }
}
\end{lstlisting} 
& Y \\[-6ex]
\hline
% __________________________________________________________
CQ7 & Which images have annotations classified under the role of "detected emotion" with an annotation strength exceeding 0.85, and what labels have been assigned to them? & \begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?Image ?Label
WHERE {
  ?Image a :Image .
  ?Annotation :aboutAnnotatedEntity ?Image ;
              :isClassifiedBy :detected_emotion ;
              :hasAnnotationStrength ?AnnotationStrength ;
              :annotationWithLexicalEntry ?LE .
  ?LE rdfs:label ?Label .
  FILTER (?AnnotationStrength > 0.85)
}
\end{lstlisting} 
& Y \\[-6ex]
\hline
% __________________________________________________________
CQ8 & What concepts type annotations about the image with ID \textit{ARTstract\_14978}? & \begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?Concept ?AnnotationRole ?AnnotationStrength
WHERE {
    ?Annotation :aboutAnnotatedEntity :ARTstract_14978 .
    ?Annotation :isClassifiedBy ?AnnotationRole .
    ?Annotation :hasAnnotationStrength ?AnnotationStrength .
    ?Annotation :typedByConcept ?Concept .
}
\end{lstlisting} 
& Y \\[-6ex]
\hline
% __________________________________________________________
CQ9 & For each lexical entry (label) that the image with ID \textit{ARTstract\_14978} was annotated with, who was the Annotator that assigned that label? & 
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?string ?Annotator 
WHERE {
    :ARTstract_14978 :isInvolvedInAnnotationSituation ?AnnotationSituation .
    ?AnnotationSituation :involvesAnnotation ?Annotation .
    ?AnnotationSituation :involvesAnnotator ?Annotator .
    ?Annotation :aboutAnnotatedEntity :ARTstract_14978.
    ?Annotation :annotationWithLexicalEntry ?LexicalEntry .
    ?LexicalEntry rdfs:label ?string .
}
\end{lstlisting} 
& Y \\[-8ex]
\hline
% __________________________________________________________
CQ10 & What types of annotations about the image with ID \textit{ARTstract\_14978} were all done by artificial annotators with the \textit{visual transformer} model architecture? & \begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?AnnotationClass ?Annotator ?Dataset
WHERE {
    ?AnnotationSituation :involvesAnnotation ?Annotation .
    ?AnnotationSituation :involvesAnnotator ?Annotator .
    ?Annotator :hasModelArchitecture :visual_transformer .
    ?Annotator :pretrainedOnDataset ?Dataset .
    ?Annotation :aboutAnnotatedEntity :ARTstract_14978 .
    ?Annotation a ?AnnotationClass .
    FILTER NOT EXISTS {
        ?subClass rdfs:subClassOf ?AnnotationClass .
        ?Annotation rdf:type ?subClass.
        FILTER (?subClass != ?AnnotationClass)
    }
}
\end{lstlisting} 
& Y \\[-8ex]
\hline
% __________________________________________________________
CQ11 & What are the caption annotations for the image with ID \textit{ARTstract\_14978}, and who are the annotators responsible for each caption annotation? & 
\begin{lstlisting}[style=sparql, xleftmargin=0.2cm]
SELECT ?Caption ?Annotator
WHERE {
  ?Annotation :aboutAnnotatedEntity :ARTstract_14978 .  
  ?Annotation a :ImageCaptionAnnotation .
  ?Annotation rdfs:comment ?Caption .
  ?AnnotationSituation :involvesAnnotation ?Annotation .
  ?AnnotationSituation :involvesAnnotator ?Annotator .
}
\end{lstlisting} 
& Y \\
\hline
\end{xtabular}
    
\caption{Competency Questions, Corresponding SPARQL Queries, and Pass Status for SituAnnotate}

\label{tab:sparql}
\end{landscape}

==> samples/extra.tex <==
% VENUE TO BE SUBMITTED TO:

% https://dl.acm.org/pb-assets/static_journal_pages/tkdd/pdf/TKDD-CfP-Trustworthy-Artificial-Intelligence.pdf

% EXTRA CONTENT FOR STATE OF THE ART:

% SemTag and seeker: bootstrapping the semantic web via automated semantic annotation
% https://dl.acm.org/doi/abs/10.1145/775152.775178

% Design and Implementation of an Ontology for Semantic Labeling and Testing: Automotive Global Ontology (AGO)
% https://www.mdpi.com/2076-3417/11/17/7782


% Hurdles to Artificial Intelligence Deployment: Noise in Schemas and “Gold” Labels
% https://pubs.rsna.org/doi/full/10.1148/ryai.220056


% Ontology-based medical image annotation with description logics
% https://ieeexplore.ieee.org/abstract/document/1250173

% A Polyvocal and Contextualised Semantic Web
% https://link.springer.com/chapter/10.1007/978-3-030-77385-4_30

% Fuzzy Annotation of Web Data Tables Driven by a Domain Ontology
% https://link.springer.com/chapter/10.1007/978-3-642-02121-3_47

% A System for Ontology-Based Annotation of Biomedical Data
% https://link.springer.com/chapter/10.1007/978-3-540-69828-9_14

% RightField: embedding ontology annotation in spreadsheets 
% https://academic.oup.com/bioinformatics/article/27/14/2021/194783
